Exploring and Benchmarking the Planning Capabilities of Large Language Models

Classical and natural language planning tasks remain a difficult domain for modern large language models (LLMs). In this work, we lay the foundations for improving planning capabilities of LLMs. First, we construct a comprehensive benchmark suite encompassing both classical planning benchmarks and natural language scenarios. This suite includes algorithms to methodically generate instances of tasks with varying levels of difficulty, allowing for rigorous and systematic evaluation of LLM performance. Next, we investigate the use of many-shot in-context learning to enhance LLM planning, exploring the relationship between increased context length and improved planning performance. In addition, we demonstrate the positive impact of fine-tuning LLMs on optimal planning paths. We also probe the efficacy of chain-of-thought reasoning methods to improve LLM planning performance. Moreover, we probe the performance of the proposed methods in out-of-distribution scenarios, assessing the ability to generalize to novel and unseen planning challenges. Finally, we investigate model's failure modes and reveal insights that hold true across different benchmarks.

==> tables/ood.tex <==


\begin{table}[htb!]
\centering
\caption{Testing Blocksworld accuracy results by model on OOD tasks.
Note for training we use in-context learning or fine-tuning.
We consider a split with problems of size 3-7 blocks and 8-9 blocks.}
\label{tab:ood-bw}
\begin{tabular}{@{\hspace{-0.0em}}lcc@{\hspace{-0.0em}}} % Adjusted spacing
\toprule
% Model Name & \multicolumn{2}{c}{Problem Size} \\
% \cmidrule(lr){2-3}
\multirow{4}{*}{Model Name} & \multicolumn{2}{c}{Train data} \\
 %\cmidrule(lr){2-3}
 &  (3 - 7) &  (8 - 9) \\
  \cmidrule(lr){2-3}
   & \multicolumn{2}{c}{Eval data} \\
   &  (3 - 7) /  (8 - 9) & (3 - 7) /  (8 - 9) \\
% &\multicolumn{2}{c}{Eval data } \\
% & \multicolumn{2}{c}{ (3 - 7) /  (8 - 9) }\\
\midrule
G 1.5 Flash (1 Shot) & 26.4 / 13.7 & 32.9  / 12.3 \\
G 1.5 Flash (70 Shot) & 35.7 / 23.3 & 27.6  / 11.0 \\
G 1.5 Pro (1 Shot) & 40.0 /  25.6 & 39.0  / 20.3 \\
G 1.5 Pro (70 Shot) & 46.3 /  36.3 & 38.3  / 18.4 \\ 
G 1.0 S (1 Shot) & 3.68 / 0.331 & 2.99   / 1.35 \\
G 1.0 S (70 Shot) & 12.4 / 2.33 & 3.99   / 1.68 \\
G 1.0 S (SFT) & 96.3 / 81.6 & 93.1   / 94.2 \\
T5 XXL (SFT) & 88.5 / 13.0  & 11.8/ 74.2 \\ 
\bottomrule
\end{tabular}
\end{table}

\begin{table}[htb!]
\centering
\caption{Testing Logistics accuracy results by model on OOD tasks.
Note for training we use in-context learning or fine-tuning.
We consider a split with problems of \kevin{1-2} and \kevin{3-5}}
\label{tab:ood-logistics}
\begin{tabular}{@{\hspace{-0.0em}}lcc@{\hspace{-0.0em}}} % Adjusted spacing
\toprule
% Model Name & \multicolumn{2}{c}{Problem Size} \\
% \cmidrule(lr){2-3}
\multirow{4}{*}{Model Name} & \multicolumn{2}{c}{Train data} \\
 %\cmidrule(lr){2-3}
 &  (1 - 2) &  (3 - 5) \\
  \cmidrule(lr){2-3}
   & \multicolumn{2}{c}{Eval data} \\
   &  (1 - 2) /  (3 - 5) & (1 - 2) /  (3 - 5) \\
% &\multicolumn{2}{c}{Eval data } \\
% & \multicolumn{2}{c}{ (3 - 7) /  (8 - 9) }\\
\midrule
G 1.5 Flash (1 Shot) & 18.3 /  1.35 & 26.7 / 1.00 \\
G 1.5 Flash (70 Shot) & 12.7 /  1.67 & 19.7  / 1.33 \\
G 1.5 Pro (1 Shot) & 35.3 / 9.03 & 57.6  / 7.01 \\
G 1.5 Pro (70 Shot) & 56.4 / 11.3 & 62.7  / 8.04 \\
G 1.0 S (1 Shot) & 7.00 / 0.000 & 5.33 / 0.000 \\
G 1.0 S (70 Shot) & 9.99 / 0.336 & 3.99  8.00 / 0.662 \\
G 1.0 S (SFT) & 99.8 / 10.8 & 98.0 / 63.4 \\
T5 XXL (SFT) & 98.4 / 7.20  & 47.4/ 5.08 \\ 
\bottomrule
\end{tabular}
\end{table}

% \begin{table}[hbt!] 
% \caption{\small Plan generalization analysis for Logistics scenarios with different number of packets in SFT scenarios, for T5 XXL, Gemini S. accuracy is measured by verifier. Acc. (in $\%$) }
% \label{tab:plan-generalization-logistic}
% \begin{center}
% \begin{tabular}{l|l|l|l} \toprule
% Finetune data & Eval data &  T5 XXL & Gemini S \\ \hline
%  Logis(1-2) & Logis(1-2) & 98.40 & 99.80 \\
%  Logis(1-2) & Logis(3-5) & 7.20 & 10.80\\
%  Logis(3-5) & Logis(1-2) & 47.40 & 98.00 \\
%  Logis(3-5) & Logis(3-5) & 5.08 & 63.40\\ \bottomrule
% \end{tabular}
% %\vspace{-15pt}
% \end{center}
% \end{table}

